Tight Reference Frame--Independent Quantum Teleportation

We give a tight scheme for teleporting a quantum state between two parties whose reference frames are misaligned by an action of a finite symmetry group. Unlike previously proposed schemes, ours requires no additional tokens or data to be passed between the participants; the same amount of classical information is transferred as for ordinary quantum teleportation, and the Hilbert space of the entangled resource is of the same size. In the terminology of Peres and Scudo, our protocol relies on classical communication of unspeakable information.

==> eptcsdata.tex <==
\providecommand{\firstpage}{202}
\providecommand{\publicationstatus}{R. Duncan and C. Heunen (Eds.): Quantum Physics and Logic (QPL) 2016\\
EPTCS 236, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.236.13}{10.4204/EPTCS.236.13}}
\pdfoutput=1

